Markets Beyond Nash Welfare for Leontief Utilities

We study the allocation of divisible goods to competing agents via a market mechanism, focusing on agents with Leontief utilities. The majority of the economics and mechanism design literature has focused on \emph{linear} prices, meaning that the cost of a good is proportional to the quantity purchased. Equilibria for linear prices are known to be exactly the maximum Nash welfare allocations. \emph{Price curves} allow the cost of a good to be any (increasing) function of the quantity purchased. We show that price curve equilibria are not limited to maximum Nash welfare allocations with two main results. First, we show that an allocation can be supported by strictly increasing price curves if and only if it is \emph{group-domination-free}. A similarly characterization holds for weakly increasing price curves. We use this to show that given any allocation, we can compute strictly (or weakly) increasing price curves that support it (or show that none exist) in polynomial time. These results involve a connection to the \emph{agent-order matrix} of an allocation, which may have other applications. Second, we use duality to show that in the bandwidth allocation setting, any allocation maximizing a CES welfare function can be supported by price curves.

==> other_CES.tex <==
\subsection{Other settings where the maximum CES welfare allocation be supported}\label{sec:ces-other}

In this section, we give two other settings where any maximum CES welfare allocation be supported: (1) when there are two agents and their weights have the same $L_q$ norm for any single $q \ge 1$ or the same $L_\infty$ norm (Theorem~\ref{thm:ces-n=2}), and (2) for any number of agents when $\sum_{j \in M} w_{ij}^\rho = 1$ for every agent $i$ (Theorem~\ref{thm:ces-rho-mean}).

Theorem~\ref{thm:ces-n=2} implies the CES welfare allocation can be supported exactly when agents' weights are $L_\infty$ normed. This is in contrast to max-min welfare (for any number of agents), where the best we can could do under the $L_\infty$ norm was an arbitrarily close approximation. In fact, the only way the norm is used in the proof of Theorem~\ref{thm:ces-n=2} is to show that if $\A\succ\succ_k \B$ (without loss of generality, say $\A$ contains only agent 1 and $\B$ contains only agent 2), then $u_1(x_1) \ge u_2(x_2)$. One imagines that this property would hold for any reasonable norm.

\begin{theorem}\label{thm:ces-n=2}
Let $n=2$, and suppose that either (1) there exists $q\geq 1$ such that $\sum_{j \in M} w_{ij}^q = 1$ for both $i \in \{1,2\}$, or (2) $\max_{j \in M} w_{ij} = 1$ for both $i \in \{1,2\}$. Then for any $\rho < 0$, every maximum CES welfare allocation can be supported by price curves. 
%\reyna{I think this holds for $n=3$ too... worth mentioning? also for literally \emph{any} norm.}
\end{theorem}

\begin{proof}
We use Lemma~\ref{lem:give-delta}. Let $\x$ be a maximum CES welfare allocation, and suppose for the sake of contradiction that $\x$ cannot be supported by price curves: then Theorem~\ref{thm:laf} implies that $\x$ is not LAF, so by Lemma~\ref{lem:laf-sgd}, there exists $\A, \B \in \bbr_{\geq 0}^n$ where $\A\succ\succ_k\B$ for some agent $k$.

We can assume without loss of generality that $\min(a_i, b_i) = 0$ for both $i \in \{1,2\}$. By symmetry, assume that $a_1 = b_2 > 0$ and $a_2 = b_1 = 0$. This means that $\A$ only contains agent 1 and $\B$ only contains agent 2. In order to apply Lemma~\ref{lem:give-delta}, we need only show that $\sum_{i \in N} (a_i - b_i) u_i(x_i)^\rho \leq 0$. In our case, this is equivalent to $u_1(x_1)^\rho \leq u_2(x_2)^\rho$, which is in turn equivalent to $u_1(x_1) \geq u_2(x_2)$.

Recall that for all $j \in M$, $x_{ij} = u_i(x_i) w_{ij}$. Since $\A \succ\succ_k \B$, $x_{1j} \geq x_{2j}$ for all $j$, which implies $u_1(x_1) w_{1j} \geq u_2(x_2) w_{2j}$. Thus either $u_1(x_1) \geq u_2(x_2)$ or $w_{1j} > w_{2j}$ for all $j$. However, if agent 1's weight vector is strictly larger than agent 2's on \emph{every} coordinate, they clearly cannot have the same $L_q$ norm for any $q$, which contradicts the assumption.

%We now proceed by cases.

%Case 1: There exists $q\geq 1$ such that $\sum_{j \in M} w_{ij}^q = 1$ for both $i \in \{1,2\}$. We know that for all $j \in M$, $u_1(x_1) = x_{1j}/w_{1j}$ and $u_2(x_2) = x_{2j}/w_{2j}$. Applying Lemma~\ref{lem:gdf-strictly-monotone} with $g(x) = x^q$ gives us $x_{1j}^q - x_{2j}^q \ge 0$ for all $j \in M$, where the inequality is strict for $j \in M_k$. Summing over all $j \in M$ gives us
%\[
%\sum_{j \in M} x_{1j}^q - \sum_{j \in M} x_{2j}^q > 0
%\]
%Also,
%\[
%\sum_{j \in M} x_{1j}^q - \sum_{j \in M} x_{2j}^q  = u_1(x_1)^q \sum_j w_{1j}^q - u_2(x_2)^q \sum_j w_{2j}^q = u_1(x_1)^q - u_2(x_2)^q
%\]
%Thus $u_1(x_1)^q - u_2(x_2)^q > 0$, and so $u_1(x_1) > u_2(x_2)$.

%Case 2: $\max_{j \in M} w_{ij} = 1$ for both $i \in \{1,2\}$. When $\max_{j \in M} w_{ij} = 1$, we have $u_i(x_i) = \max_{j \in M} x_{ij}$. The definition of $\A\succ\succ_k\B$ implies that $x_{1j} \geq x_{2j}$ for all $j \in M_k$. Thus $\max_{j \in M} x_{1j} \geq \max_{j \in M} x_{2j}$, which implies that $u_1(x_1) \geq u_2(x_2)$.

%Thus $u_1(x_1) > u_2(x_2)$ in either case, and so $\sum_{i \in N} (a_i - b_i) u_i(x_i)^\rho < 0$ (although we did not need the inequality to be strict). Therefore by Lemma~\ref{lem:give-delta}, $\x$ cannot be a maximum CES welfare allocation, which is a contradiction.
\end{proof}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{theorem}\label{thm:ces-rho-mean}
Suppose that $w_{ij} > 0$ for all $i \in N$ and $j \in M$, $\rho < 0$, and $\sum_{j \in M} w_{ij}^\rho = 1$ for all $i \in N$. Then any maximum CES welfare allocation can be supported by price curves.
\end{theorem}

\begin{proof}
We again use Lemma~\ref{lem:give-delta}. Let $\x$ be a maximum CES welfare allocation that cannot be supported by price curves: then Theorem~\ref{thm:laf} implies that $\x$ is not LAF, so by Lemma~\ref{lem:laf-sgd}, there exists $\A, \B \in \bbr_{\geq 0}^n$ where $\A\succ\succ_k\B$ for some agent $k$. 

Since $\rho < 0$, $g(x) = x^\rho$ is a strictly decreasing function. Thus by Lemma~\ref{lem:gdf-decreasing}, for all $j \in M$ we have $\sum_{i \in N} (a_i - b_i) x_{ij}^\rho \le 0$, and for each $j \in M_k$, the inequality is strict. Summing over all $j \in M$ gives us
\[
\sum_{j\in M} \sum_{i \in N} (a_i - b_i) x_{ij}^\rho < 0
\]

We again have $x_{ij} = u_i(x_i) w_{ij}$, and so
\begin{align*}
\sum_{j \in M} \sum_{i \in N} (a_i - b_i) x_{ij}^\rho =&\ \sum_{j \in M} \sum_{i \in N} (a_i - b_i) u_i(x_i)^\rho w_{ij}^\rho\\
=&\ \sum_{i \in N} (a_i - b_i) u_i(x_i)^\rho \sum_{j \in M} w_{ij}^\rho \\
=&\ \sum_{i \in N} (a_i - b_i) u_i(x_i)^\rho
\end{align*}

Therefore $\sum_{i \in N} (a_i - b_i) u_i(x_i)^\rho < 0$, so Lemma~\ref{lem:give-delta} applies, and this shows that any maximum CES allocation can be supported by price curves.
\end{proof}
